Biathlon: Harnessing Model Resilience for Accelerating ML Inference Pipelines

Machine learning inference pipelines commonly encountered in data science and industries often require real-time responsiveness due to their user-facing nature. However, meeting this requirement becomes particularly challenging when certain input features require aggregating a large volume of data online. Recent literature on interpretable machine learning reveals that most machine learning models exhibit a notable degree of resilience to variations in input. This suggests that machine learning models can effectively accommodate approximate input features with minimal discernible impact on accuracy. In this paper, we introduce Biathlon, a novel ML serving system that leverages the inherent resilience of models and determines the optimal degree of approximation for each aggregation feature. This approach enables maximum speedup while ensuring a guaranteed bound on accuracy loss. We evaluate Biathlon on real pipelines from both industry applications and data science competitions, demonstrating its ability to meet real-time latency requirements by achieving 5.3x to 16.6x speedup with almost no accuracy loss.

==> elements_in_template.tex <==

\section{Core Structural Elements}
\subsection{Figures}
\autoref{fig:duck}.

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/duck}
  \caption{An illustration of a Mallard Duck. Picture from Mabel Osgood Wright, \textit{Birdcraft}, published 1897.}
  \label{fig:duck}
\end{figure}

\begin{table*}[t]
  \caption{A double column table.}
  \label{tab:commands}
  \begin{tabular}{ccl}
    \toprule
    A Wide Command Column & A Random Number & Comments\\
    \midrule
    \verb|\tabular| & 100& The content of a table \\
    \verb|\table|  & 300 & For floating tables within a single column\\
    \verb|\table*| & 400 & For wider floating tables that span two columns\\
    \bottomrule
  \end{tabular}
\end{table*}

\subsection{Tables}
\autoref{tab:commands}.
\autoref{tab:freq}. 

\begin{table}[hb]% h asks to places the floating element [h]ere.
  \caption{Frequency of Special Characters}
  \label{tab:freq}
  \begin{tabular}{ccl}
    \toprule
    Non-English or Math & Frequency & Comments\\
    \midrule
    \O & 1 in 1000& For Swedish names\\
    $\pi$ & 1 in 5 & Common in math\\
    \$ & 4 in 5 & Used in business\\
    $\Psi^2_1$ & 1 in 40\,000 & Unexplained usage\\
  \bottomrule
\end{tabular}
\end{table}

\subsection{Listings and Styles}
\subsection{Math and Equations}

\begin{equation}
  \lim_{n\rightarrow \infty}x=0
\end{equation}

\begin{displaymath}
  \sum_{i=0}^{\infty} x + 1
\end{displaymath}

\begin{equation}
  \sum_{i=0}^{\infty}x_i=\int_{0}^{\pi+2} f
\end{equation}


\section{Citations}

Some examples of references. A paginated journal article~\cite{Abril07}, an enumerated journal article~\cite{Cohen07}, a reference to an entire issue~\cite{JCohen96}, a monograph (whole book) ~\cite{Kosiur01}, a monograph/whole book in a series (see 2a in spec. document)~\cite{Harel79}, a divisible-book such as an anthology or compilation~\cite{Editor00} followed by the same example, however we only output the series if the volume number is given~\cite{Editor00a} (so Editor00a's series should NOT be present since it has no vol. no.), a chapter in a divisible book~\cite{Spector90}, a chapter in a divisible book in a series~\cite{Douglass98}, a multi-volume work as book~\cite{Knuth97}, an article in a proceedings (of a conference, symposium, workshop for example) (paginated proceedings article)~\cite{Andler79}, a proceedings article with all possible elements~\cite{Smith10}, an example of an enumerated proceedings article~\cite{VanGundy07}, an informally published work~\cite{Harel78}, a doctoral dissertation~\cite{Clarkson85}, a master's thesis~\cite{anisi03}, an finally two online documents or world wide web resources~\cite{Thornburg01, Ablamowicz07}.

==> extra_workload_table.tex <==
\begin{table}[]
\centering
\resizebox{1.1\columnwidth}{!}{
\hspace*{-1cm}
\begin{tabular}{|c|c||cccc||cc||c|}
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}} Pipeline \\(Description) \end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}} DataSet (Num \\ of Records)\end{tabular}} &
  \multicolumn{4}{c|}{Num of Operators} &
  \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Num of\\ Features\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Num of\\ User\\ Requests\end{tabular}} \\ \cline{3-8}
   &
   &
  \multicolumn{2}{c|}{Datastore} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Transfor \\ -mation\end{tabular}}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Model\\ Inference\end{tabular}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{AGG}}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Non-\\ AGG\end{tabular}} &
   \\ \cline{3-4}
   &
   &
  \multicolumn{1}{c|}{\textbf{AGG}} &
  \multicolumn{1}{c|}{Others} &
  \multicolumn{1}{c|}{} &
   &
  \multicolumn{1}{c|}{} &
   &
   \\ \hline\hline
\begin{tabular}[c]{@{}c@{}}Trip-Fare \cite{trips-feast}\\ (Predict fare \\ of a trip)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}NYC \\ Taxi \cite{NYC-Dataset} (3B)\end{tabular} &
  \multicolumn{1}{c|}{2} &
  \multicolumn{1}{c|}{0} &
  \multicolumn{1}{c|}{5} &
  \begin{tabular}[c]{@{}c@{}} LGBM \\ (Regression)\end{tabular} &
  \multicolumn{1}{c|}{3} &
  5 &
  400 \\ \hline
\begin{tabular}[c]{@{}c@{}}Tick-Price \cite{tick-lr}\\ (Forecast price\\  of a tick)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Forex \\ Tick \cite{Forex-Tick} (1.1B)\end{tabular} &
  \multicolumn{1}{c|}{1} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{0} &
  \begin{tabular}[c]{@{}c@{}} LR \\ (Regression)\end{tabular} &
  \multicolumn{1}{c|}{1} &
  6 &
  516 \\ \hline
\begin{tabular}[c]{@{}c@{}}Bearing-Imbalance \\ \cite{Bearing}(Detect \\ Imbalance of bearing)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Machinery \\ Fault \cite{Machinery-Fault} (95M)\end{tabular} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{0} &
  \multicolumn{1}{c|}{0} &
  \begin{tabular}[c]{@{}c@{}} MLP \\ (Classification)\end{tabular} &
  \multicolumn{1}{c|}{8} &
  0 &
  338 \\ \hline
\begin{tabular}[c]{@{}c@{}}Fraud-Detection \cite{tdfraud}\\ (Detect fraudulent\\ click of user)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}TalkingData Click\\  \cite{TalkingData-Clicklog} (242M)\end{tabular} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{0} &
  \multicolumn{1}{c|}{6} &
  \begin{tabular}[c]{@{}c@{}} MLP \\ (Classification)\end{tabular} &
  \multicolumn{1}{c|}{3} &
  6 &
  500 \\ \hline
\end{tabular}
}
\caption*{Table 1*: Extra Inference Pipelines}
\vspace{-3em}
\label{tab:extra-workload}
\end{table}
